Revisiting the Graph Reasoning Ability of Large Language Models: Case Studies in Translation, Connectivity and Shortest Path

Large Language Models (LLMs) have achieved great success in various reasoning tasks. In this work, we focus on the graph reasoning ability of LLMs. Although theoretical studies proved that LLMs are capable of handling graph reasoning tasks, empirical evaluations reveal numerous failures. To deepen our understanding on this discrepancy, we revisit the ability of LLMs on three fundamental graph tasks: graph description translation, graph connectivity, and the shortest-path problem. Our findings suggest that LLMs can fail to understand graph structures through text descriptions and exhibit varying performance for all these three fundamental tasks. Meanwhile, we perform a real-world investigation on knowledge graphs and make consistent observations with our findings. The codes and datasets are available.

==> latex/05_theories.tex <==
% \section{Possible Explanations behind the discrepancy}

% \subsection{Inherent mechanism within LLMs}
% \noindent \textbf{Hallucination:} First of all, some failure cases are possibly caused by faithfulness hallucination, i.e., LLMs tend to generate content logically inconsistent to the input and the instruction. For instance, in the tasks of graph description translation, LLMs occasionally ignore some edges or introduce non-existent edges, diverging from the input. \xn{shown in appendix} Since the translation tasks do not need complex reasoning, these errors are mainly from the mixture of training data. LLMs recall and blend graphs from their training data with the current input graph.
% This phenomenon can also be observed in the way node IDs affect the outcome. We mentioned that an increased risk of failure in LLMs when we assign random numbers or characters to node IDs, compared with sequentially ordered ones. Such randomness in node IDs diverges from the common patterns found in the training data of LLMs, thereby triggering textual hallucinations. 
%\jt{how about the prediction and the output path inconsistency in the graph connectivity task? }


\noindent \textbf{Non-general shortcuts:} Secondly, there could exist some shortcuts to help LLMs in conducting graph reasoning. Take a singleton as an instance. We observed that LLMs consistently succeed with singleton, which is independent on the difficulty of the graph questions.
%\jt{please check the following adding content and please revise if necessary:  which is independent on the complexity and hardness of the graph.} 
This suggests that LLMs have learned a shortcut: nodes not mentioned in the edge description are considered isolated. 
However, this shortcut is not a general rule for LLMs to solve graph problems. It only works when the target nodes are isolated, which does not adapt to other situations.
% However, shortcuts are not always correct. If 
% LLMs rely on the rule of non-mentioned edges to solve other situations, it will lead to errors.\xn{When?}


% \noindent \textbf{Influence of auto-aggressive loss:} Thirdly, 
% %\jt{to be careful, I think we should say the LLMs we choose to test are} \jt{add references to support} 
% most transformer-based LLMs are pretrained by next token prediction and some spurious correlations are introduced. 
% The training dataset 
% %\jt{are you sure the pretraining data contains graphs?? please give some evidence to support} {currently no, we need to finetune LLMs by some graphs to verify it.}
% consists of various graphs with their reachable paths. The adoption of an auto-aggressive loss function facilitates the emergence of a frequency-based spurious correlation, enabling the prediction of next node ID based on preceding node IDs within the path. This logic is different from the value-based \xn{cite?} state update mechanism to find the reachable path, thereby influencing the LLMs' ability to deduce accurate answers.
% Moreover, the issue becomes severer as the length of the reachable path increases, ultimately emerging as the primary reason behind the decline performance of LLMs' graph reasoning.


% \subsection{Impact of different graph descriptions }

% The various graph descriptions influence the time complexity of LLMs to conduct a certain algorithm, and the time complexity represent the difficulty of the algorithm to some extent. 
% %\jt{how time complexity affects the performance??} 
% However, the previous theoretical work overlooked this difference. Here we take breath-first search as an example to carefully examine it on the two graph descriptions, Edge List and Node List. 

%the framework of the decision-making problem built by the previous theoretical work (described in Section \ref{basic_theory}) is incomplete compared with the actual calculation procedure taken by LLMs. Based on our experimental results, we propose a new process and analyze the time complexity of depth-first search as example, on the two graph descriptions, edge lists and node lists. 

%Suppose that the edge lists are represented by $\{(v_i, v_j)\}_{|E|}$, and the node lists are denoted as $\{(v_i, \{u_{i1}, u_{i2}, u_{i3}\}_{|N_{v_i}|})\}_{|N|}$, \jt{throughout the paper, we use different notations to denote the number of edges and nodes, let us make them consistent. We could define them in 2.4 and then directly use them in the following sections} where $|E|$ is the total number of edges and $|N_{v_i}|$ indicates the number of neighbors for node $v_i$ within the set of all nodes, denoted by $|N|$. 
% We define these two descriptions in Section \ref{basic_theory}. When LLMs conduct BFS, LLMs should maintain two arrays to represent a state, a queue storing nodes pending exploration and a visited set including visited nodes. Thus, LLMs at most process $N$ states. However, when LLMs update the state, they need different efforts based on different descriptions. For the node lists, it is easy to find all the positions of neighbor nodes, which costs $\mathcal{O}(|N|)$. However, it takes  $\mathcal{O}(|E|)$ for edge lists. Therefore, the overall algorithmic complexity is different, where the node lists should be $\mathcal{O}(|N|^2)$ while the edge lists should be $\mathcal{O}(|N||E|)$. 




%Despite the classical graph reasoning tasks can be formulated as dynamic programming, which can be done in LLMs shown in \ref{basic_theory}, the calculation progress can be different when inputting a string into LLMs. We take the DFS algorithm on the directed graph as an example and show them 



%The pseudo-code of new processes for DFS is provided in Appendix \ref{algs}.


%Here, the latent space can be any other data structure, such as a queue in BFS and transition space for dynamic functions according to \cite{feng2024towards}. Therefore, the algorithm complex is different in practical, where the Node List should be $\mathcal{O}(N^2+kN^2)$ while Edge List should be $\mathcal{O}(N+kN_E^2)$. K means the k-hop step for the detection, which can not be ignored in the graph reasoning tasks. The formulation suggests that there is a gap between the ideal algorithms applications and the practical algorithms. The increasing of $k$,$N$, and $N_E$ can lead to an increase in computational complexity for LLMs. Besides, the LLMs may meet the bottleneck while the computational complexity increases \cite{xu2024hallucination}.

==> latex/tables/acc_table.tex <==
% \begin{table}[]
%     \centering
%     \small
% \begin{tabular}{cccccc}
% Des. & Models & Tiny & Easy & Med. & Hard \\
% \multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{GraphInstruct}} \\
% \multirow{2}{*}{ \textbf{Node} } & GPT-3 & 0.7950 & 0.7906 & 0.7427 & 0.6981 \\
% & GPT-4 & 0.9734 & 0.8514 & 0.7251 & 0.6981 \\
% \multirow{2}{*}{ \textbf{Edge} } & GPT-3 & 0.7863 & 0.777 & 0.7309 & 0.7358 \\
% & GPT-4 & 0.9734 & 0.8582 & 0.8889 & 0.7799 \\
% \multicolumn{2}{c}{} & \multicolumn{4}{c}{\textbf{NLGraph}} \\
% \multirow{2}{*}{ \textbf{Node} } & GPT-3 & - & 0.7443 & 0.6592 & 0.6500 \\
% & GPT-4 & - & 0.9375 & 0.7933 & 0.7706 \\
% \multirow{2}{*}{ \textbf{Edge} } & GPT-3 & - & 0.8807 & 0.7875 & 0.7279 \\
% & GPT-4 & - & 0.9830 & 0.8958 & 0.8838 \\
% \end{tabular}
%     \caption{The performance of LLMs on the graph connectivity task. We use the accuracy metrics for the evaluations. The datasets are categorized to different difficulties as Tiny, Easy, Medium and Hard according to the graph node number.}
%     \label{acc_table}
% \end{table}


% \begin{table}[]
%     \centering
%     \small
%     \setlength{\tabcolsep}{6pt}
% \begin{tabular}{cc|cccccccccc}
% \toprule
% \multirow{2}{*}{ Des. } & \multirow{2}{*}{ Models } & \multicolumn{2}{c}{Tiny} & \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Med} & \multicolumn{2}{c}{Hard} \\
% & & ACC & $\mathrm{F_{acc}}$ & ACC & $\mathrm{F_{acc}}$ & ACC & $\mathrm{F_{acc}}$ & ACC & $\mathrm{F_{acc}}$ \\
% \midrule
% \multicolumn{2}{c|}{Dataset} & \multicolumn{8}{c}{GraphInstruct} \\
% \multirow{2}{*}{ Node } & GPT-3 & 0.93 & 0.92 & 0.79 & 0.75 & 0.69 & 0.67 & 0.71 & 0.63 \\
% & GPT-4 & 0.99 & 0.99 & 0.97 & 0.95 & 0.96 & 0.89 & 0.90 & 0.83 \\
% \multirow{2}{*}{ Edge } & GPT-3 & 0.91 & 0.87 & 0.75 & 0.66 & 0.68 & 0.57 & 0.70 & 0.51 \\
% & GPT-4 & 1.00 & 0.98 & 0.99 & 0.97 & 0.98 & 0.95 & 0.96 & 0.89 \\
% \midrule
% \multicolumn{2}{c|}{Dataset} & \multicolumn{8}{c}{NLGraph} \\
% \multirow{2}{*}{ Node } & GPT-3 & - & & 0.7443 & & 0.6592 & & 0.65 & \\
% & GPT-4 & - & & 0.9375 & & 0.7933 & & 0.7706 & \\
% \multirow{2}{*}{ Edge } & GPT-3 & - & & 0.8807 & & 0.7875 & & 0.7279 & \\
% & GPT-4 & - & & 0.983 & & 0.8958 & & 0.8838 & \\
% \bottomrule
% \end{tabular}
%     \caption{The performance of LLMs on the graph connectivity task. We use the accuracy metrics for the evaluations. The datasets are categorized to different difficulties as Tiny, Easy, Medium and Hard according to the graph node number.}
%     \label{acc_table}
% \end{table}


\begin{table}[]
    \centering
    \tiny
    \setlength{\tabcolsep}{10pt}
\begin{tabular}{@{\hskip 0in}c@{\hskip 0in}c@{\hskip 0in}c@{\hskip 0in}c|cccc}
\toprule
Dataset & Models & Des. & & Tiny & Small & Med & Hard \\
\midrule
\multirow{8}{*}{ Undirected } & \multirow{4}{*}{ GPT-3 } & \multirow{2}{*}{ Node } & ACC & 0.93 & 0.79 & 0.68 & 0.71 \\
& & & $\mathrm{F_{acc}}$ & 0.92 & 0.75 & 0.66 & 0.63 \\
& & \multirow{2}{*}{ Edge } & ACC & 0.91 & 0.75 & 0.68 & 0.70 \\
& & & $\mathrm{F_{acc}}$ & 0.87 & 0.66 & 0.57 & 0.51 \\
& \multirow{4}{*}{ GPT-4 } & \multirow{2}{*}{ Node } & ACC & 0.99 & 0.92 & 0.86 & 0.79 \\
& & & $\mathrm{F_{acc}}$ & 0.99 & 0.90 & 0.79 & 0.72 \\
& & \multirow{2}{*}{ Edge } & ACC & 0.99 & 0.94 & 0.93 & 0.88 \\
& & & $\mathrm{F_{acc}}$ & 0.97 & 0.92 & 0.90 & 0.81 \\
\midrule
\multirow{8}{*}{ Directed } & \multirow{4}{*}{ GPT-3 } & \multirow{2}{*}{ Node } & ACC & 0.20 & 0.17 & 0.19 & 0.32 \\
& & & $\mathrm{F_{acc}}$ & 0.06 & 0.03 & 0.07 & 0.14 \\
& & \multirow{2}{*}{ Edge } & ACC & 0.25 & 0.28 & 0.32 & 0.37 \\
& & & $\mathrm{F_{acc}}$ & 0.22 & 0.26 & 0.22 & 0.26 \\
& \multirow{4}{*}{ GPT-4 } & \multirow{2}{*}{ Node } & ACC & 0.90 & 0.90 & 0.74 & 0.70 \\
& & & $\mathrm{F_{acc}}$ & 0.90 & 0.89 & 0.68 & 0.60 \\
& & \multirow{2}{*}{ Edge } & ACC & 0.88 & 0.86 & 0.75 & 0.76 \\
& & & $\mathrm{F_{acc}}$ & 0.88 & 0.84 & 0.70 & 0.70 \\
\bottomrule
\end{tabular}
    \caption{The performance of LLMs on the graph connectivity task. We use the accuracy metrics for the evaluations. The datasets are categorized to different difficulties as Tiny, Easy, Medium and Hard according to the graph node number.}
    \label{acc_table}
\end{table}

==> latex/tables/baseline_results.tex <==
\begin{table}[]
    \centering
    \tiny
    \setlength{\tabcolsep}{3pt}
\begin{tabular}{cc|cccccccc}
\toprule
\multirow{2}{*}{ Des. } & \multirow{2}{*}{ Models } & \multicolumn{2}{c}{Tiny} & \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Med} & \multicolumn{2}{c}{Hard} \\
& & ACC & $\mathrm{F_{acc}}$ & ACC & $\mathrm{F_{acc}}$ & ACC & $\mathrm{F_{acc}}$ & ACC & $\mathrm{F_{acc}}$ \\
\midrule
\multicolumn{2}{c|}{Dataset} & \multicolumn{8}{c}{GraphInstruct} \\
\multirow{2}{*}{ Node } & GPT-3 & 0.93 & 0.92 & 0.79 & 0.75 & 0.69 & 0.67 & 0.71 & 0.63 \\
& GPT-4 & 0.99 & 0.99 & 0.97 & 0.95 & 0.96 & 0.89 & 0.90 & 0.83 \\
\multirow{2}{*}{ Edge } & GPT-3 & 0.91 & 0.87 & 0.75 & 0.66 & 0.68 & 0.57 & 0.70 & 0.51 \\
& GPT-4 & 1.00 & 0.98 & 0.99 & 0.97 & 0.98 & 0.95 & 0.96 & 0.89 \\
\bottomrule
\end{tabular}
    \caption{Results of GraphInstruct}
    \label{baseline_results}
\end{table}

==> latex/tables/parameters.tex <==
\begin{table}[]
\small
    \centering
        \caption{The GPT-2 parameters}
\begin{tabular}{lllll}
\toprule
            & \# Params & \multicolumn{1}{l}{\# head} & \multicolumn{1}{l}{\# layer} & \multicolumn{1}{l}{\# emb} \\
            \midrule
Baby-GPT2   & 80M        & 6                            & 6                             & 384                         \\
Small-GPT2  & 124M       & 12                           & 12                            & 768                         \\
Medium-GPT2 & 350M       & 24                           & 16                            & 1024  \\
\bottomrule
\end{tabular}
\end{table}

==> latex/tables/strategy3.tex <==
\begin{table}[]
    \centering
    \small
\begin{tabular}{ccccc}
Subdataset & \multicolumn{2}{c}{0-BF} & \multicolumn{2}{c}{0-FW} \\
Des. & Node & Edge & Node & Edge \\
1<k<2 hops & & & & \\
3<k<4 hops & & & & \\
5-hops & & & & \\
Singleton & & & & \\
Isolated C. & & & & \\
Asymmetric & & & & \\
AVG. & & & & \\
\end{tabular}
    \caption{Caption}
    \label{stratage_3}
\end{table}
